BigDetection: A Large-scale Benchmark for Improved Object Detector Pre-training

Multiple datasets and open challenges for object detection have been introduced in recent years. To build more general and powerful object detection systems, in this paper, we construct a new large-scale benchmark termed BigDetection. Our goal is to simply leverage the training data from existing datasets (LVIS, OpenImages and Object365) with carefully designed principles, and curate a larger dataset for improved detector pre-training. Specifically, we generate a new taxonomy which unifies the heterogeneous label spaces from different sources. Our BigDetection dataset has 600 object categories and contains over 3.4M training images with 36M bounding boxes. It is much larger in multiple dimensions than previous benchmarks, which offers both opportunities and challenges. Extensive experiments demonstrate its validity as a new benchmark for evaluating different object detection methods, and its effectiveness as a pre-training dataset.

==> figs/classes_merging.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=0.9\linewidth]{images/bird_class_merging.png}
  \caption{Example of producing the ``\textit{bird}'' class in BigDetection using classes merging.}
  \label{fig:classes_merging}
\end{figure}

==> tables/self-training.tex <==
\begin{table}[t]
    %\renewcommand\arraystretch{1.2}
    \begin{center}
        \begin{tabular}{cc|cccc}
            \toprule
            score thr & nms thr & AP & AP$_{50}$ & AP$_{75}$ & COCO \\
            \midrule
            - & - & \textbf{23.1} & \textbf{30.2} & \textbf{24.9} & 45.3 \\
            \midrule
            0.4 & 0.7 & 21.1 & 27.8 & 22.7 & 45.5 \\
            0.5 & 0.7 & 22.1 & 29.0 & 23.7 & 45.6 \\
            0.6 & 0.7 & 22.6 & 29.6 & 24.3 & 45.5 \\
            \midrule
            0.5 & 0.5 & 22.0 & 28.8 & 23.6 & 45.5 \\
            0.5 & 0.6 & 22.1 & 28.9 & 23.7 & \textbf{45.7} \\
            \bottomrule
        \end{tabular}
    \end{center}
    \caption{Ablation study on the effect of different hyperparameters for generating pseudo labels.}
    \label{tab:self-training}
\end{table}
